Friction-adaptive descent: a family of dynamics-based optimization methods

We describe a family of descent algorithms which generalizes common existing schemes used in applications such as neural network training and more broadly for optimization of smooth functions--potentially for global optimization, or as a local optimization method to be deployed within global optimization schemes like basin hopping. By introducing an auxiliary degree of freedom we create a dynamical system with improved stability, reducing oscillatory modes and accelerating convergence to minima. The resulting algorithms are simple to implement and control, and convergence can be shown directly by Lyapunov's second method. Although this framework, which we refer to as friction-adaptive descent (FAD), is fairly general, we focus most of our attention here on a specific variant: kinetic energy stabilization (which can be viewed as a zero-temperature Nos\'e--Hoover scheme but with added dissipation in both physical and auxiliary variables), termed KFAD (kinetic FAD). To illustrate the flexibility of the FAD framework we consider several other methods. in certain asymptotic limits, these methods can be viewed as introducing cubic damping in various forms; they can be more efficient than linearly dissipated Hamiltonian dynamics in common optimization settings. We present details of the numerical methods and show convergence for both the continuous and discretized dynamics in the convex setting by constructing Lyapunov functions. The methods are tested using a toy model (the Rosenbrock function). We also demonstrate the methods for structural optimization for atomic clusters in Lennard--Jones and Morse potentials. The experiments show the relative efficiency and robustness of FAD in comparison to linearly dissipated Hamiltonian dynamics.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{mathrsfs}
\usepackage{enumerate}
\usepackage{todonotes}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Friction-adaptive descent}{ Karoni, K., Leimkuhler, B. and Stoltz, G.}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Friction-adaptive descent: a family of dynamics-based optimization methods\thanks{Submitted to the editors 26-4-2023.
\funding{The work of KK and BL was funded by the Engineering
and Physical Sciences Research Council Grant EP/S023291/1 (MAC-MIGS Centre
for Doctoral Training) and EP/R014604/1 (Isaac Newton Institute), specifically funding provided by its Data-Driven Engineering programme (Spring 2023).
The work of GS was funded by the European Research Council (ERC) under the European Union's Horizon 2020 research and innovation programme (project EMC2, grant agreement No 810367), and by Agence Nationale de la Recherche, under grants ANR-19-CE40-0010-01 (QuAMProcs) and ANR-21-CE40-0006 (SINEQ).}}}

% Authors: full names plus addresses.
 \author{Katerina Karoni\thanks{School of Mathematics, University of Edinburgh, Edinburgh EH9 2NX} \and Benedict Leimkuhler  \footnotemark[3]\and Gabriel Stoltz \thanks{CERMICS, Ecole des Ponts, Marne-la-Vall\'ee, France, \& MATHERIALS team-project, Inria Paris,France}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

